LiDAR-Generated Images Derived Keypoints Assisted Point Cloud Registration Scheme in Odometry Estimation

Keypoint detection and description play a pivotal role in various robotics and autonomous applications including visual odometry (VO), visual navigation, and Simultaneous localization and mapping (SLAM). While a myriad of keypoint detectors and descriptors have been extensively studied in conventional camera images, the effectiveness of these techniques in the context of LiDAR-generated images, i.e. reflectivity and ranges images, has not been assessed. These images have gained attention due to their resilience in adverse conditions such as rain or fog. Additionally, they contain significant textural information that supplements the geometric information provided by LiDAR point clouds in the point cloud registration phase, especially when reliant solely on LiDAR sensors. This addresses the challenge of drift encountered in LiDAR Odometry (LO) within geometrically identical scenarios or where not all the raw point cloud is informative and may even be misleading. This paper aims to analyze the applicability of conventional image key point extractors and descriptors on LiDAR-generated images via a comprehensive quantitative investigation. Moreover, we propose a novel approach to enhance the robustness and reliability of LO. After extracting key points, we proceed to downsample the point cloud, subsequently integrating it into the point cloud registration phase for the purpose of odometry estimation. Our experiment demonstrates that the proposed approach has comparable accuracy but reduced computational overhead, higher odometry publishing rate, and even superior performance in scenarios prone to drift by using the raw point cloud. This, in turn, lays a foundation for subsequent investigations into the integration of LiDAR-generated images with LO. Our code is available on GitHub: https://github.com/TIERS/ws-lidar-as-camera-odom.

==> tbs/res-result.tex <==
\begin{table}[!ht]
    \centering
    \caption{Evaluation metrics under different image sizes.}
    \label{tab:analysis-of-resize}
    \resizebox{\textwidth}{!}
    {
    \begin{tabular}{ccccccc}
    \hline
        \textbf{Interpolation} & \textbf{Size} & \textbf{Robustness of rotation} & \textbf{Robustness of scaling} & \textbf{Robustness with noise} & \textbf{Distinctiveness} & \textbf{Matching Score} \\ \hline
        ~ & 512x32 & 0.859/0.008 & 0.166/0.006 & 0.547/0.068 & 0.253/0.05 & 0.373/0.09 \\ 
        ~ & 896x128 & 0.825/0.007 & 0.162/0.006 & 0.585/0.022 & 0.364/0.016 & 0.511/0.009 \\ 
        ~ & 896x256 & 0.847/0.011 & 0.147/0.006 & 0.666/0.012 & 0.305/0.013 & 0.484/0.016 \\ 
        ~ & \textbf{1024x64} & \textbf{0.808/0.015} & \textbf{0.125/0.004} & \textbf{0.533/0.029} & \textbf{0.431/0.018} & \textbf{0.535/0.005} \\ 
        ~ & 1024x128 & 0.83/0.007 & 0.151/0.006 & 0.58/0.022 & 0.373/0.016 & 0.505/0.008 \\ 
        ~ & 1024x256 & 0.854/0.009 & 0.135/0.006 & 0.661/0.012 & 0.319/0.014 & 0.484/0.015 \\ 
        ~ & 1280x64 & 0.796/0.018 & 0.119/0.004 & 0.513/0.028 & 0.411/0.017 & 0.502/0.006 \\ 
        CUBIC & 1280x128 & 0.819/0.007 & 0.144/0.006 & 0.567/0.023 & 0.35/0.015 & 0.478/0.008 \\ 
        ~ & 1280x256 & 0.853/0.01 & 0.129/0.006 & 0.655/0.013 & 0.298/0.013 & 0.461/0.016 \\ 
        ~ & 1920x128 & 0.806/0.008 & 0.129/0.005 & 0.549/0.024 & 0.318/0.013 & 0.434/0.008 \\ 
        ~ & 1920x256 & 0.853/0.01 & 0.117/0.006 & 0.65/0.014 & 0.269/0.011 & 0.429/0.017 \\ 
        ~ & 2048x128 & 0.799/0.008 & 0.129/0.006 & 0.544/0.027 & 0.309/0.013 & 0.425/0.009 \\ 
        ~ & 2048x256 & 0.844/0.01 & 0.118/0.006 & 0.637/0.015 & 0.26/0.011 & 0.42/0.018 \\ 
        ~ & 2560x128 & 0.803/0.009 & 0.115/0.005 & 0.543/0.026 & 0.293/0.011 & 0.399/0.01 \\ 
        ~ & 2560x256 & 0.855/0.011 & 0.109/0.006 & 0.654/0.015 & 0.246/0.01 & 0.401/0.019 \\ 
        ~ & 4096x128 & 0.795/0.01 & 0.084/0.004 & 0.556/0.037 & 0.256/0.008 & 0.337/0.011 \\ \midrule
        ~ & 512x32 & 0.858/0.008 & 0.178/0.007 & 0.538/0.065 & 0.245/0.048 & 0.367/0.087 \\ 
        ~ & 896x128 & 0.825/0.007 & 0.164/0.006 & 0.583/0.021 & 0.358/0.017 & 0.508/0.009 \\ 
        ~ & 896x256 & 0.85/0.01 & 0.154/0.007 & 0.666/0.012 & 0.295/0.013 & 0.478/0.017 \\ 
        ~ & \textbf{1024x64} & \textbf{0.803/0.015} & \textbf{0.136/0.004} & \textbf{0.518/0.028} & \textbf{0.417/0.019} & \textbf{0.527/0.006} \\ 
        ~ & 1024x128 & 0.825/0.006 & 0.156/0.006 & 0.571/0.023 & 0.366/0.017 & 0.5/0.008 \\ 
        ~ & 1024x256 & 0.855/0.009 & 0.142/0.006 & 0.654/0.013 & 0.31/0.014 & 0.476/0.016 \\ 
        ~ & 1280x64 & 0.789/0.018 & 0.13/0.004 & 0.502/0.028 & 0.401/0.018 & 0.498/0.006 \\ 
        LANCZOS4 & 1280x128 & 0.814/0.007 & 0.147/0.006 & 0.561/0.024 & 0.349/0.015 & 0.478/0.008 \\ 
        ~ & 1280x256 & 0.852/0.009 & 0.136/0.006 & 0.646/0.014 & 0.295/0.013 & 0.463/0.017 \\ 
        ~ & 1920x128 & 0.8/0.008 & 0.133/0.006 & 0.541/0.025 & 0.316/0.013 & 0.433/0.008 \\ 
        ~ & 1920x256 & 0.85/0.01 & 0.124/0.006 & 0.639/0.014 & 0.265/0.011 & 0.428/0.018 \\ 
        ~ & 2048x128 & 0.799/0.008 & 0.129/0.006 & 0.544/0.027 & 0.309/0.013 & 0.425/0.009 \\ 
        ~ & 2048x256 & 0.845/0.01 & 0.124/0.006 & 0.632/0.015 & 0.257/0.011 & 0.421/0.018 \\ 
        ~ & 2560x128 & 0.799/0.009 & 0.12/0.005 & 0.533/0.025 & 0.29/0.011 & 0.396/0.01 \\ 
        ~ & 2560x256 & 0.855/0.011 & 0.115/0.006 & 0.642/0.015 & 0.241/0.01 & 0.398/0.019 \\ 
        ~ & 4096x128 & 0.794/0.01 & 0.088/0.004 & 0.551/0.039 & 0.251/0.009 & 0.333/0.011 \\ \midrule
        ~ & 512x32 & 0.853/0.008 & 0.115/0.005 & 0.578/0.076 & 0.321/0.072 & 0.357/0.099 \\ 
        ~ & 896x128 & 0.835/0.009 & 0.136/0.004 & 0.612/0.02 & 0.401/0.015 & 0.536/0.006 \\ 
        ~ & 896x256 & 0.839/0.01 & 0.147/0.005 & 0.659/0.013 & 0.32/0.013 & 0.494/0.011 \\ 
        ~ & \textbf{1024x64} & \textbf{0.814/0.015} & \textbf{0.103/0.003} & \textbf{0.559/0.029} & \textbf{0.455/0.016} & \textbf{0.542/0.005} \\ 
        ~ & 1024x128 & 0.839/0.007 & 0.135/0.004 & 0.599/0.022 & 0.386/0.016 & 0.513/0.007 \\ 
        ~ & 1024x256 & 0.849/0.009 & 0.131/0.005 & 0.662/0.013 & 0.333/0.013 & 0.496/0.011 \\ 
        ~ & 1280x64 & 0.807/0.018 & 0.092/0.003 & 0.552/0.029 & 0.442/0.015 & 0.514/0.005 \\ 
        AREA & 1280x128 & 0.834/0.007 & 0.122/0.004 & 0.595/0.022 & 0.373/0.014 & 0.49/0.007 \\ 
        ~ & 1280x256 & 0.846/0.009 & 0.124/0.005 & 0.656/0.013 & 0.312/0.012 & 0.473/0.011 \\ 
        ~ & 1920x128 & 0.815/0.008 & 0.113/0.004 & 0.567/0.025 & 0.332/0.012 & 0.442/0.008 \\ 
        ~ & 1920x256 & 0.838/0.01 & 0.11/0.005 & 0.646/0.014 & 0.282/0.01 & 0.436/0.013 \\ 
        ~ & 2048x128 & 0.799/0.008 & 0.129/0.006 & 0.544/0.027 & 0.309/0.013 & 0.425/0.009 \\ 
        ~ & 2048x256 & 0.826/0.01 & 0.125/0.006 & 0.624/0.017 & 0.263/0.011 & 0.42/0.013 \\ 
        ~ & 2560x128 & 0.8/0.009 & 0.105/0.004 & 0.551/0.027 & 0.3/0.011 & 0.405/0.009 \\ 
        ~ & 2560x256 & 0.827/0.01 & 0.104/0.005 & 0.634/0.017 & 0.253/0.009 & 0.403/0.014 \\ 
        ~ & 4096x128 & 0.809/0.014 & 0.098/0.004 & 0.557/0.043 & 0.25/0.008 & 0.336/0.011 \\ \midrule
        ~ & 512x32 & 0.851/0.008 & 0.182/0.008 & 0.533/0.063 & 0.237/0.045 & 0.358/0.084 \\ 
        ~ & 896x128 & 0.821/0.007 & 0.164/0.006 & 0.579/0.022 & 0.352/0.016 & 0.503/0.009 \\ 
        ~ & 896x256 & 0.838/0.01 & 0.16/0.006 & 0.652/0.014 & 0.293/0.013 & 0.477/0.012 \\ 
        ~ & \textbf{1024x64} & \textbf{0.807/0.018} & \textbf{0.152/0.005} & \textbf{0.531/0.025} & \textbf{0.379/0.018} & \textbf{0.505/0.008} \\ 
        ~ & 1024x128 & 0.827/0.006 & 0.157/0.006 & 0.571/0.024 & 0.35/0.017 & 0.489/0.009 \\ 
        ~ & 1024x256 & 0.845/0.008 & 0.15/0.006 & 0.643/0.015 & 0.293/0.013 & 0.466/0.013 \\ 
        ~ & 1280x64 & 0.799/0.02 & 0.141/0.005 & 0.526/0.025 & 0.363/0.017 & 0.478/0.007 \\ 
        NEAREST & 1280x128 & 0.822/0.007 & 0.146/0.006 & 0.57/0.025 & 0.335/0.015 & 0.466/0.009 \\ 
        ~ & 1280x256 & 0.84/0.009 & 0.141/0.006 & 0.636/0.015 & 0.28/0.012 & 0.453/0.013 \\ 
        ~ & 1920x128 & 0.803/0.008 & 0.132/0.006 & 0.545/0.027 & 0.309/0.013 & 0.429/0.009 \\ 
        ~ & 1920x256 & 0.83/0.01 & 0.127/0.006 & 0.624/0.017 & 0.262/0.011 & 0.425/0.013 \\ 
        ~ & 2048x128 & 0.799/0.008 & 0.129/0.006 & 0.544/0.027 & 0.309/0.013 & 0.425/0.009 \\ 
        ~ & 2048x256 & 0.826/0.01 & 0.125/0.006 & 0.624/0.017 & 0.263/0.011 & 0.42/0.013 \\ 
        ~ & 2560x128 & 0.801/0.009 & 0.12/0.005 & 0.545/0.03 & 0.283/0.011 & 0.393/0.009 \\ 
        ~ & 2560x256 & 0.824/0.01 & 0.117/0.006 & 0.622/0.018 & 0.237/0.009 & 0.396/0.015 \\ 
        ~ & 4096x128 & 0.809/0.014 & 0.098/0.004 & 0.557/0.043 & 0.25/0.008 & 0.336/0.011 \\ \midrule
        ~ & 512x32 & 0.858/0.009 & 0.146/0.005 & 0.559/0.071 & 0.281/0.059 & 0.376/0.09 \\ 
        ~ & 896x128 & 0.828/0.008 & 0.152/0.005 & 0.594/0.021 & 0.376/0.016 & 0.519/0.008 \\ 
        ~ & 896x256 & 0.843/0.011 & 0.124/0.006 & 0.671/0.013 & 0.333/0.013 & 0.495/0.013 \\ 
        ~ & \textbf{1024x64} & \textbf{0.814/0.015} & \textbf{0.103/0.003} & \textbf{0.559/0.029} & \textbf{0.455/0.016} & \textbf{0.542/0.005} \\ 
        ~ & 1024x128 & 0.838/0.007 & 0.135/0.004 & 0.598/0.022 & 0.386/0.016 & 0.513/0.007 \\ 
        ~ & 1024x256 & 0.854/0.009 & 0.11/0.005 & 0.674/0.014 & 0.344/0.013 & 0.494/0.013 \\ 
        ~ & 1280x64 & 0.802/0.017 & 0.099/0.003 & 0.54/0.027 & 0.431/0.016 & 0.51/0.006 \\ 
        LINEAR & 1280x128 & 0.827/0.007 & 0.131/0.005 & 0.583/0.023 & 0.36/0.015 & 0.482/0.008 \\ 
        ~ & 1280x256 & 0.851/0.01 & 0.106/0.005 & 0.665/0.014 & 0.319/0.013 & 0.468/0.015 \\ 
        ~ & 1920x128 & 0.814/0.008 & 0.114/0.004 & 0.565/0.025 & 0.33/0.012 & 0.441/0.008 \\ 
        ~ & 1920x256 & 0.849/0.01 & 0.092/0.005 & 0.663/0.015 & 0.291/0.011 & 0.434/0.015 \\ 
        ~ & 2048x128 & 0.799/0.008 & 0.129/0.006 & 0.544/0.027 & 0.309/0.013 & 0.425/0.009 \\ 
        ~ & 2048x256 & 0.843/0.011 & 0.102/0.006 & 0.649/0.016 & 0.274/0.011 & 0.422/0.017 \\ 
        ~ & 2560x128 & 0.806/0.009 & 0.098/0.004 & 0.562/0.027 & 0.307/0.011 & 0.407/0.009 \\ 
        ~ & 2560x256 & 0.847/0.011 & 0.087/0.005 & 0.666/0.018 & 0.269/0.01 & 0.406/0.016 \\ 
        ~ & 4096x128 & 0.789/0.011 & 0.068/0.003 & 0.563/0.037 & 0.277/0.008 & 0.35/0.01 \\ \bottomrule
    \end{tabular}
    }
\end{table}






